Consistent and Flexible Selectivity Estimation for High-Dimensional Data

Selectivity estimation aims at estimating the number of database objects that satisfy a selection criterion. Answering this problem accurately and efficiently is essential to many applications, such as density estimation, outlier detection, query optimization, and data integration. The estimation problem is especially challenging for large-scale high-dimensional data due to the curse of dimensionality, the large variance of selectivity across different queries, and the need to make the estimator consistent (i.e., the selectivity is non-decreasing in the threshold). We propose a new deep learning-based model that learns a query-dependent piecewise linear function as selectivity estimator, which is flexible to fit the selectivity curve of any distance function and query object, while guaranteeing that the output is non-decreasing in the threshold. To improve the accuracy for large datasets, we propose to partition the dataset into multiple disjoint subsets and build a local model on each of them. We perform experiments on real datasets and show that the proposed model consistently outperforms state-of-the-art models in accuracy in an efficient way and is useful for real applications.

==> method_wasted.tex <==
% !TeX root = body/ARN.tex

\section{Proposed Approach}

\subsection{Overview}

Let $y = f(\xx, t)$ denote the selectivity (in absolute scale) of the query
$\xx$ and threshold $t$ against a static database of objects. We call this
function $f$ the \textbf{value function}. 





\subsection{Data Parttition}

%% motivation
When the database size is large, it is hard to estimate $f$ directly. One of the
main challenges is that $f$ may be non-smooth.

In the worst case, $f$ is not sufficiently ``smooth'' with respect to both input
parameters.
%% put them as Lemma? 
\begin{itemize}
\item For any $\epsilon > 0$, there exist a database of $n$ objects and a query
  $(\xx, t)$ such that $f(\xx, t) = 0$ and $f(\xx + \epsilon, t) = n$.
\item For any $\epsilon > 0$, There exist a database of $n$ objects and a query
  $(\xx, t)$ such that $f(\xx, t) = 0$ and $f(\xx, t+\epsilon) = n$.
\end{itemize}
%% need logic and support
This means any model that directly approximate $f$ is hard.

In this paper, we propose to decompose the database into disjoint partitions,
such that we can approximate the value functions on each partitions individually
and then sum up the estimates as the final estimate.

For any partition of the DB into $w$ partitions, we denote the value functions
defined on the partition $f_i$. Our final estimate will be
$\sum_{i=1}^w \est{f}_i(\xx; t)$.


\paragraph{Merged Cover Tree}

%% overview
This is done in three steps.

In the first step, we create fine-grained partitions using the Cover Tree
algorithm~\cite{covertree}. Given a shrinking parameter $\alpha$, the Cover Tree
construction algorithm recursively divide the dataset into non-empty partitions,
each with a radius of at most $\frac{1}{\alpha}$ than the radius of the current
dataset. 

The leaf partitions obtained the Cover Tree are typically heavily skewed. In
addition, the number of partitions tend to be large. These characteristics will
affect the accuracy of the model built for each partitions, and increase the
model size and training time, respectively. 

Hence, as the second step, we merge the leaf partitons such that:
\begin{inparaenum}[(i)]
\item the partition sizes are less skewed, and 
\item the total number of partitions is $w$, as specified by the user.
\end{inparaenum}
We found that different partition merging algorithm have minimal impact on the
quality and efficiency of our method. Therefore, we just adopt a simple greedy
algorithm as shown in Algorithm~\cite{alg:merge-partitions}. 

%% explain the alg
The algorithm ...

%%======================================================================
\begin{algorithm}
  \small%
  \State{$\mathcal{Q} \gets \emptyset$}
  \State{$\mathcal{P} \gets$ leaf partitions of the Cover Tree in decreasing sizes}
  \ForEach{partiton $P \in \mathcal{P}$}{
    \State{xxx}
  }
  \Return{$Q$}
  %% 
  \caption{\algMergePartitions($\mathcal{P}$, $w$)}\label{alg:merge-partitions}
\end{algorithm}
%%======================================================================

As the final step, we maintain the sub-partitions in a merged partition to their
corresponding ones in the Cover Tree. We term the final Cover Tree the merged
Cover Tree\fixme{better name?}. 

\paragraph{Learning Partition-specific Estimateion Model}

The data 



\paragraph{Estimateion Algorithm}

Our design can be deemed as a special case of the Learned Index proposal
optimized for the estimatieon task. An ensemble of machine learning models are
built, and one or multiple models are invoked to jointly complete a task. The
major difference is that the key decision of which models need to be invoked at
each step in~\cite{learned-index} is determined by a decision model, in our
case, we have a simpler and lossless method instead. 




\paragraph{Pruning Partitions}

If the selection predict of the query satisfy some properties, and we keep
certain statistics about each partitions, it is possible to \emph{prune} the
partitions. There are two cases for the pruning a partition $P$:
\begin{itemize}
\item [Case I] $\lbd(P, q) > t$: this mean all objects in $P$ are more than $t$ distance
  from $q$. Hence, this partition can be pruned as its contribution to the final
  estimate is guaranteed to be 0.
\item [Case II] $\ubd(P, q) \leq t$: : this mean all objects in $P$ are no more than $t$
  distance from $q$. Hence, this partition can be pruned as its contribution to
  the final estimate is guaranteed to be $|P|$\footnote{i.e., we only need to
    access the meta information kept for all partitions.}.
\end{itemize}

One example is when the predicate is a metric distance (such as $l_2$ distance
for real vectors and edit distances for strings). For each partition $P$, we can
compute a representative object $c(P)$, and the radius of the partition centered
at $c(P)$ (denoted as $r(P)$). This partition can be pruned for Cases I and II
if $t \geq d(c(P), \xx) + r(P)$ and $t < d(c(P), \xx) - r(P)$, respectively.

As another example, we can accommodate Ptolemaic distances, such as the
\emph{signature quadratic form distance} used in multimedia
databases~\cite{SISAP11}\fixme{Ptolemaic Indexing of the Signature Quadratic
  Form Distance [SISAP11]}. We need to select two representative objects for
every partition, and similar pruning conditions can be derived following the
Ptolemaic's inequality. 







%\subsection{Test \LaTeX{} Macros}
%
%$\argmin_{\Btheta} \ell(f(\xx_i; \Btheta), y_i)$
%
%%%!! important comments are written using the prefix: %%!!
%\fixme{To be removed later.}
%
%\cite{bgf:Lixto}
 
 


%%!! DO NOT DELETE the following block

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> sigmodblock.tex <==
{\fontsize{8pt}{8pt} \selectfont
\textbf{ACM Reference Format:}\\
Yaoshu Wang, Chuan Xiao, Jianbin Qin, Rui Mao, Makoto Onizuka, Wei Wang, Rui Zhang, and Yoshiharu Ishikawa. 2021. Consistent and Flexible Selectivity Estimation for High-Dimensional Data. In {\it Proceedings of the 2021 International Conference on Management of Data (SIGMOD ’21), June 20--25, 2021, Virtual Event, China.} ACM, New York, NY, USA, 9 pages. https://doi.org/10.1145/3448016.3452772}


==> vldbblock.tex <==
%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\begingroup\small\noindent\raggedright\textbf{PVLDB Reference Format:}\\
\vldbauthors. \vldbtitle. PVLDB, \vldbvolume(\vldbissue): \vldbpages, \vldbyear.\\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi}
\endgroup
\begingroup
\renewcommand\thefootnote{}\footnote{\noindent
This work is licensed under the Creative Commons BY-NC-ND 4.0 International License. Visit \url{https://creativecommons.org/licenses/by-nc-nd/4.0/} to view a copy of this license. For any use beyond those covered by this license, obtain permission by emailing \href{mailto:info@vldb.org}{info@vldb.org}. Copyright is held by the owner/author(s). Publication rights licensed to the VLDB Endowment. \\
\raggedright Proceedings of the VLDB Endowment, Vol. \vldbvolume, No. \vldbissue\ %
ISSN 2150-8097. \\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi} \\
}\addtocounter{footnote}{-1}\endgroup
%%% VLDB block end %%%
